Asynchronous Complex Analytics in a Distributed Dataflow Architecture

Scalable distributed dataflow systems have recently experienced widespread adoption, with commodity dataflow engines such as Hadoop and Spark, and even commodity SQL engines routinely supporting increasingly sophisticated analytics tasks (e.g., support vector machines, logistic regression, collaborative filtering). However, these systems' synchronous (often Bulk Synchronous Parallel) dataflow execution model is at odds with an increasingly important trend in the machine learning community: the use of asynchrony via shared, mutable state (i.e., data races) in convex programming tasks, which has---in a single-node context---delivered noteworthy empirical performance gains and inspired new research into asynchronous algorithms. In this work, we attempt to bridge this gap by evaluating the use of lightweight, asynchronous state transfer within a commodity dataflow engine. Specifically, we investigate the use of asynchronous sideways information passing (ASIP) that presents single-stage parallel iterators with a Volcano-like intra-operator iterator that can be used for asynchronous information passing. We port two synchronous convex programming algorithms, stochastic gradient descent and the alternating direction method of multipliers (ADMM), to use ASIPs. We evaluate an implementation of ASIPs within on Apache Spark that exhibits considerable speedups as well as a rich set of performance trade-offs in the use of these asynchronous algorithms.

==> admm.tex <==

\section{A Principled Baseline: ADMM}
\label{sec:ADMM}

As a starting point for our \system coordination algorithms, we adapt
a classic algorithm called Alternating Direction Method of Multipliers
(ADMM). In this section, we provide a gentle introduction to ADMM and
discuss its behavior in light of the characteristics discussed in
Section~\ref{sec:goodproperties}.

\subsection{ADMM Intuition and Basics}

The Alternating Direction Method of Multipliers (ADMM) is one of the
most robust distributed convex programming methods in the literature
(\cite{boyd-admm}~provides an excellent technical survey). Adapted to
the \system framework from Section~\ref{sec:architecture}, 

To understand how exactly to determine $\overline{x}^k$ and
$\lambda^k$, we have to consider the second ``step'' in each ADMM
round: the \textit{dual update}. ADMM takes its ``Alternating'' name
because it repeatedly alternates between solving the primal update and
solving this second, dual update step. In the dual update
step, ADMM first updates the consensus variable by taking the average of
all local solutions $x_k$ from the previous round:
$$\overline{x}^{k+1} = \sum_{i=1}^n \frac{x_i}{n}$$
Subsequently, ADMM updates the Lagrangian variable:
$$\lambda^{k+1} = \lambda^k + \rho(x_i^{k+1} - \overline{x}^{k+1})$$
Overall, ADMM repeats these two-step rounds indefinitely until
convergence, which can be determined by either periodically
calculating the value of the objective function, or, alternatively, by
tracking the rate of change (the \textit{residual}) of each of the
local solvers.

We can consider using ADMM (and later, do and evaluate) as baseline
implementation of \system coordination. In a \naive BSP-based
implementation, \system would begin by initializing the consensus and
Lagrangian variables to zero, then successively invoke a series of
primal followed by dual updates. First, \system would invoke each
local solver on the appropriately-formatted primal step. Second, after
waiting for all of the local solvers to terminate, \system would
collect the results and perform the dual step, averaging the primal
results to update the consensus and subsequently calculating the
Lagrangian variable. \system would repeat this process until
convergence. Figure~\ref{fig:bsp-comm} provides an illustration of
this computation and communication pattern between local solvers.


\begin{figure*}

\subfigure[Traditional ADMM]{
\includegraphics[width=.3679\linewidth]{figs/bsp-comm.pdf}
\label{fig:bsp-comm}
}
\hfill
\subfigure[\minibatch]{
\includegraphics[width=.2691\linewidth]{figs/minibatch-comm.pdf}
\label{fig:minibatch-comm}
}
\hfill
\subfigure[\async] {
\includegraphics[width=.2276\linewidth]{figs/async-comm.pdf}
\label{fig:async-comm}
}

\caption{Communication patterns for ADMM, \minibatch, and \async
  algorithms for three local solvers. Time runs from left to right,
  with barriers illustrated as vertical black bars and local
  computation as colored blocks. ADMM uses generic BSP-style
  primal-dual rounds, while \minibatch limits the duration of each
  primal solve using a timeout. \async removes all barriers, allowing
  asynchronous primal and dual solves as well as sharing of solver
  results.}
\end{figure*}

The use of ADMM exhibits several attractive properties. Foremost,
ADMM is stable and achieves good convergence rates without many
assumptions. It requires a convex objective (more precisely, primal
and dual feasibility) but guarantees convergence despite data and
performance variance across local solvers. In the event of no
statistically significant variance across solvers, ADMM reduces to
distributed averaging and will return after one iteration. In the
event of data skew, ADMM will run more iterations but will eventually
complete. Moreover, ADMM does not depend on timing assumptions for
correctness---individual processes might have to wait for stragglers,
but the algorithm will, with eventual delivery, eventually make
progress. Finally, ADMM is---as far as distributed optimization
algorithms are concerned---relatively simple. This may be surprising,
especially given the seeming mysticism of the Lagrangian term, but, as
far as implementation complexity is concerned, ADMM is a manageable
solution.

Readers familiar with the Escrow technique~\cite{escrow} or the
Demarcation protocol~\cite{demarcation} from transaction processing
systems might benefit from thinking of ADMM in these terms. Both
Escrow and Demarcation ``partition,'' or rewrite, a global, linear
constraint such that a set of processes can independently operate
without violating the global constraint simply by checking their local
constraint linear (e.g., with $N$ processes, we could rewrite $x < k$
as $x < \frac{k}{N}$). ADMM similarly partitions the solution space
between processes and allows them to move within this space, but
careful modifies the local constraints (here, objective functions) to
bound the degree of divergence. However, unlike Escrow and
Demarcation, which completely disallow the global system state to
violate the fixed constraint, ADMM uses the quadratic penalty
associated with its consensus term to impose a non-fixed but otherwise
stabilizing local penalty for deviation (namely, the square of the
norm).

\subsection{ADMM Overheads}

\label{sec:admm-limitations}

While ADMM provides robust execution and is---from a pragmatic
perspective---a reasonably simple starting point for distributed
convex programming, it is not a panacea. There are three primary
concerns that we will address in order to provide more efficient and
practical implementation of \system.

First, ADMM solves each local primal subproblem entirely before
sharing results (in the form of local solutions). This provides
stability but can be slow. In particular, each local process solves
its local problem without any knowledge of the concurrently executing
processes. This provides solutions that, on a per-process basis, are
sound. However, to guarantee that solutions are a good fit globally,
each solver must wait until every other solver has completed
solving. In the event that all solvers agree, their local solver will
reach a point where they cannot make progress due to the consensus
term (i.e., the quadratic the penalty for deviating from the
average). To recompute the new average, they must communicate. In the
event that solvers disagree, they may solve their own local
subproblems and, only after they have completed their solves will they
realize that they may have individually ``wasted'' work by operating
under a stale Lagrangian term. In theoretical analysis, these
overheads drop out as constant terms in the asymptotic limits; in
practical settings, as we demonstrate, they are a barrier to efficient
execution.

Second, ADMM is inherently a synchronous algorithm is therefore
subject to the effects of stragglers and performance variance between
solvers. The success of the asynchronous learning mechanisms (at least
in SMP settings) suggests that there is an opportunity to extract
additional performance by introducing asynchrony and reducing
synchronous barriers from execution.

Finally, it is unclear how well ADMM behaves in practice in modern
cluster compute frameworks. Despite the large amount of theoretical
interest in the algorithm, we are aware of only two experimental
evaluations of distributed implementations in the literature based on
custom (MPI~\cite{boyd-admm} and C++~\cite{zhang-async-admm})
implementations and both operating over synthetic datasets. Whether
ADMM's convergence guarantees translate to real-world performance
gains in a distributed setting is unproven in the literature, and we
are unaware of any actual integration into a modern data-parallel
distributed analytics framework. Some of the core proponents of ADMM
have noted that ``the fact that ADMM was developed so far in advance
of the ready availability of large-scale distributed computing systems
and massive optimization problems may account for why it is not as
widely known today as we believe it should be''~\cite{admm}

To address the first two concerns, we modify the core ADMM technique
in the next section. To address the final concern, we implement
(Section~\ref{sec:implementation}) and evaluate ADMM (along with our
other algorithms and several existing algorithms;
Section~\ref{sec:evaluation}) in a modern cluster computing framework.
 

\begin{comment}

In this paper, we start with a safe and robust algorithm and make it
faster, by reducing barriers and encouraging more fine-grained
communciation between distributed workers. This allows us to retain
the benefits of stable and understandable execution while, when
possible, extracting greater efficiency from the structure of the
underlying process.

As our baseline solution, we turn to a decades-old algorithm called
ADMM. In a sense, this is the ``serializability'' of distributed
optimization: guaranteed to work, but with---as we
discuss---performance penalties. 

At a high level, traditionally, ADMM is a BSP-style coordination of
individual solver processes. ADMM lets individual solver processes run
independently to completion while adding additional constraints to the
objective function to ensure processors do not diverge
indefinitely. Given a local solver routine and an objective function,
ADMM augments the objective function with the two terms.

The first, the consensus term, ensures that processors do not stray
too far. This is like having each processor on an elastic band.

The second, the lagrangian term, describes the shape of the solution
depending on the previous global consensus. Deep theory here, but
actually pretty simple (show an example):

ADMM proceeds iteratively in two steps: solve the local subproblem,
then, based on the local solutions, solve the lagrangian and repeat
until convergence. Intuition as to why this is stable.

The downside of ADMM is that the dependency on local solves has two
costs. First, can result in wasted or even misdirected computation
while each local process works within a round without benefiting from
useful remote information. In the limit, this is fine, but, in
practice, this wasted work can lead to substantial
inefficiency. Second, as in all of BSP prone to stragglers.

Unfortunately, there has been little study of ADMM in commodity
cluster compute frameworks or at scale. There is a large amount of
exciting theory on the problem, but its empirical properties are
largely unknown. One contribution of this paper---in addition to
addressing the above two problems---is to actually quantify the
overheads of ADMM coordination.

\end{comment}
